Few-Shot Visual Question Generation: A Novel Task and Benchmark Datasets

Generating natural language questions from visual scenes, known as Visual Question Generation (VQG), has been explored in the recent past where large amounts of meticulously labeled data provide the training corpus. However, in practice, it is not uncommon to have only a few images with question annotations corresponding to a few types of answers. In this paper, we propose a new and challenging Few-Shot Visual Question Generation (FS-VQG) task and provide a comprehensive benchmark to it. Specifically, we evaluate various existing VQG approaches as well as popular few-shot solutions based on meta-learning and self-supervised strategies for the FS-VQG task. We conduct experiments on two popular existing datasets VQG and Visual7w. In addition, we have also cleaned and extended the VQG dataset for use in a few-shot scenario, with additional image-question pairs as well as additional answer categories. We call this new dataset VQG-23. Several important findings emerge from our experiments, that shed light on the limits of current models in few-shot vision and language generation tasks. We find that trivially extending existing VQG approaches with transfer learning or meta-learning may not be enough to tackle the inherent challenges in few-shot VQG. We believe that this work will contribute to accelerating the progress in few-shot learning research.

==> ablation.tex <==
\noindent{\bf Ablation Studies:} 
Comparing the performance of our proposed approaches in different settings, we observe the following. Replacing the pre-trained Resnet-152~\cite{resnet152} feature maps with pre-trained Efficient-b3~\cite{effnet-pmlr19} feature maps, and using BERT~\cite{bert-naacl19} word embeddings instead of learning them from scratch improves models` performance,
thereby indicating that richer input features help the model learn better.
We also applied two different types of side information on our approaches -- (1)~category and (2)~answer. 
For Visual7W and VQG-23 datasets, the model  performs better with category as side-information than with answer. For VQG-16, however, the model performs better with image and answer as input as compared to that with image and category as input. This may be because of the miscategorizations in VQG-16 (described earlier) due to which the models get confused.
 
% \if 0
% \noindent{\bf Ablation Studies:} We then try to find answers to the question what influences our model most? In this regard we performed various ablation studies of our \model{}, wherein we changed the image and categories and added answers as well. More details can be found below:

% The first question that we seek answers to is does rich feature embeddings help improve the model's accuracy? In that regard, we changed the image embedding and the word embedding of \model{}. For image embedding, we used the efficient-net~\cite{effnet-pmlr19} embeddings instead of the ResNet152~\cite{resnet152} embeddings.
% For the word embeddings we used the BERT~\cite{bert-naacl19} embeddings instead of the learning embeddings from scratch. In this study we found that using rich feature embeddings does help the model achieve greater scores.

% We then evaluated as to how does the performance of VQG vary with varying inputs. In this regard, we did two specific experiments--1)replaced the input category with the answer 2)added answer. We found the accuracy of the model to improve when we replaced answer  with category as side information. 
% A reverse trend, however, can be observed in the case of VQG-16 dataset where the model with image and answer  as input performs better than the models with image and category as input. This maybe because of the conflicts in the answer category due to which the models get confused.

% An interesting observation that can be made from the results are that, the results of the \model{} on Visual7W are quite similar to that of the baseline models, unlike the results on VQG-16 and \dataset{} datasets. This may be due to the reason that the variety of questions is much less in Visual7W in comparison to that of VQG-16 and \dataset{}, resulting in the baseline models learn better even in the few-shot setting. We calculate the variety per input side-information to get a rough estimate for the above. Specifically we calculate the  ratio of number of unique question-answer pairs to number of unique answers. A high value of the ratio indicates that the variety of questions is high and vice-versa. This ratio for Visual7W is $3.014$ while that of VQG-16 and \dataset{} is $193.40$ and $517.3$ respectively.
% \fi

==> conclu.tex <==
\section{Conclusion}
% \todo{need to change}
% \vspace{-3mm}

We propose a novel few-shot VQG task and a novel attention-based model \model{} for the said task. Our proposed model outperforms several VQG models suitably adapted for the few-shot task. 
%Since there has been no prior work in few shot VQG, \model{} may serve to be a baseline for future work on few-shot VQG. 
We also propose a new dataset \dataset{}
specifically for this task, which will help evaluate future few-shot VQG models.
